Uncertainty Driven Active Learning for Image Segmentation in Underwater Inspection

Active learning aims to select the minimum amount of data to train a model that performs similarly to a model trained with the entire dataset. We study the potential of active learning for image segmentation in underwater infrastructure inspection tasks, where large amounts of data are typically collected. The pipeline inspection images are usually semantically repetitive but with great variations in quality. We use mutual information as the acquisition function, calculated using Monte Carlo dropout. To assess the effectiveness of the framework, DenseNet and HyperSeg are trained with the CamVid dataset using active learning. In addition, HyperSeg is trained with a pipeline inspection dataset of over 50,000 images. For the pipeline dataset, HyperSeg with active learning achieved 67.5% meanIoU using 12.5% of the data, and 61.4% with the same amount of randomly selected images. This shows that using active learning for segmentation models in underwater inspection tasks can lower the cost significantly.

==> sections/Experiment.tex <==
\section{Experiment}
\label{Sec:experiment}

For the experiments, the model DenseNet was selected. The datasets used were CamVid, SUIM and a private dataset composed of underwater pipelines survey videos.

==> sections/Measuring-epistemic-uncertainty.tex <==
\section{Measuring Epistemic Uncertainty}
\label{Sec:related_work}

The epistemic uncertainty can be measured using different measures when utilizing \gls{MC-Dropout}, such as variation ratio, mutual information, total variance, margin of confidence and predictive entropy. \cite{milanes2021monte} 

For explaining these five measures, consider the case of a classification problem with $\mathcal{C}$ classes, with output $p_t = (p_{1t}, ..., p_{Ct})$ for a single forward pass $t$. Consider $p^* = (p_{1}^*, ..., p_{C}^*)$ the average of $T$ forward passes using \gls{MC-Dropout}.

Considering that $c_t=arg max\{p_{1t}, ..., p_{Ct}\}$ is predicted class in the foward pass $t$, and that $c_m$ is the mode of $c_t$ for $T$ passes, the variation ratio measures the dispersion around $c_m$, and is calculated by the Equation \ref{eq:variation_ratio}:

\begin{equation} \label{eq:variation_ratio}
    \mathcal{V}_{R} = 1 -  \frac{f_{c_m}}{T}
\end{equation}

Where $f_{c_m}$ is the frequency of $c_m$, and $\mathcal{V}_{R}$ ranges from 0, when $f_{c_m}=T$, to $1/C$, when $f_{c_m}=T/C$, meaning maximum dispersion.

The total variance is calculated as Equation \ref{eq:total_variance}:

\begin{equation} \label{eq:total_variance}
    \mathcal{V}_{tot} = \frac{1}{T} \sum_{c=1}^{C}\sum_{t=1}^{T}(p_{ct}-p_c^*)^2
\end{equation}

The predictive entropy measures the amount of information in the predicted distribution and is calculated as Equation \ref{eq:predictive_entropy}, and ranges from 0 to $log_2C$.

\begin{equation} \label{eq:predictive_entropy}
    \mathcal{H} =  \sum_{c=1}^{C}p_c^*log_2(p_c^*)
\end{equation}

The mutual information can be approximately calculated as Equation \ref{eq:mutual_information}:

\begin{equation} \label{eq:mutual_information}
    \mathcal{I} = \mathcal{H} - \frac{1}{T}  \sum_{c=1}^{C}\sum_{t=1}^{T}p_{ct}log_2(p_{ct})
\end{equation}

Finally, the margin of confidence uses the difference between the two predicted values in each forward pass, as shows the Equation \ref{eq:marginOfConfidence}.

\begin{equation} \label{eq:marginOfConfidence}
    \mathcal{M} = \frac{1}{T}  \sum_{t=1}^{T}(\max p_{jt} - \max_{c \neq j} p_{ct})
\end{equation}

Where $j = arg\max p_j^*$ is the predicted class of $p^*$, obtained as the average of the predictions using \gls{MC-Dropout}.

==> sections/table_code.tex <==
\begin{table}[!htb]
\caption{CamVid Results}
\label{tab:DatasetsDetails}
\renewcommand{\arraystretch}{2}
\begin{tabular}{  | p{0.02\linewidth} | p{ 0.18\linewidth}| p{ 0.08\linewidth}| p{ 0.08\linewidth}|  p{ 0.08\linewidth} | p{ 0.08\linewidth}|  p{ 0.08\linewidth} | p{ 0.08\linewidth} |}
%\begin{tabular}{ | m{4em} | m{2cm}| m{1cm} | m{1.2cm} | m{0.7cm} | m{3cm} | m{4cm} | }


\hline
    \multicolumn{2}{|l|}{\multirow{2}{*}{Iteration}}
     &
    \multicolumn{6}{c}{ \textbf{Experiments} } \vline \\  \cline{3-8}
     
    \multicolumn{2}{|l|}{}
    &
    \textbf{Exp1} & 
    \textbf{Exp2}   &
    \textbf{Exp3} & 
    \textbf{Exp4}  &
    \textbf{Exp5}  &
    \textbf{Mean}\\

\hline 

\multirow{4}{*}{0} &
    Imgs. Train &
    36 & 
    -  &
    -  &
    - &
    - &
    - \\\cline{2-8}

     & 
    Imgs. Val &
    10   &
    - & 
    -  &
    -  &
    - &
    - \\\cline{2-8}


     & 
    mIoU &
    32.93   &
    - & 
    -  &
    -  &
    - &
    - \\
    
\hline
    

    \multirow{4}{*}{1} &
    Imgs. Train &
    68 & 
    -  &
    -  &
    - &
    - &
    - \\\cline{2-8}

     & 
    Imgs. Val &
    15   &
    - & 
    -  &
    -  &
    - &
    - \\\cline{2-8}


     & 
    mIoU - EU &
    45.47   &
    - & 
    -  &
    -  &
    - &
    - \\\cline{2-8}

      & 
    mIoU - Rand. &
    40.05   &
    - & 
    -  &
    -  &
    - &
    - \\
    
\hline

\multirow{4}{*}{2} &
    Imgs. Train &
    89 & 
    -  &
    -  &
    - &
    - &
    - \\\cline{2-8}

     & 
    Imgs. Val &
    19   &
    - & 
    -  &
    -  &
    - &
    - \\\cline{2-8}


     & 
    mIoU - EU &
    46.20   &
    - & 
    -  &
    -  &
    - &
    - \\\cline{2-8}

      & 
    mIoU - Rand. &
    44.94   &
    - & 
    -  &
    -  &
    - &
    - \\
    
\hline

\multirow{4}{*}{3} &
    Imgs. Train &
    111 & 
    -  &
    -  &
    - &
    - &
    - \\\cline{2-8}

     & 
    Imgs. Val &
    25   &
    - & 
    -  &
    -  &
    - &
    - \\\cline{2-8}


     & 
    mIoU - EU &
    48.83   &
    - & 
    -  &
    -  &
    - &
    - \\\cline{2-8}

      & 
    mIoU - Rand. &
    -   &
    - & 
    -  &
    -  &
    - &
    - \\
    
\hline

\multirow{4}{*}{

\begin{turn}{90} 
Train w. All
\end{turn}

} &
    Imgs. Train &
    367 & 
    -  &
    -  &
    - &
    - &
    - \\\cline{2-8}

     & 
    Imgs. Val &
    -   &
    - & 
    -  &
    -  &
    - &
    - \\\cline{2-8}


     & 
    mIoU &
    32.93   &
    - & 
    -  &
    -  &
    - &
    - \\
    
\hline

\end{tabular}
\end{table}

